Multi-Robot Informative Path Planning from Regression with Sparse Gaussian Processes (with Appendix)

This paper addresses multi-robot informative path planning (IPP) for environmental monitoring. The problem involves determining informative regions in the environment that should be visited by robots to gather the most information about the environment. We propose an efficient sparse Gaussian process-based approach that uses gradient descent to optimize paths in continuous environments. Our approach efficiently scales to both spatially and spatio-temporally correlated environments. Moreover, our approach can simultaneously optimize the informative paths while accounting for routing constraints, such as a distance budget and limits on the robot's velocity and acceleration. Our approach can be used for IPP with both discrete and continuous sensing robots, with point and non-point field-of-view sensing shapes, and for both single and multi-robot IPP. We demonstrate that the proposed approach is fast and accurate on real-world data.

==> ct-scan.tex <==
\subsection{Introduction}
Tomography is another important field in which one has to recover an underlying data field from integrated sensor data. The problem is often studied in computerized tomography (CT) and requires informative sensor placement~\cite{LongiRSMRSHK20}. Fugitive gas density estimation in oil fields using tunable diode laser absorption spectroscopy (TDLAS) sensors that report only the integrated gas concentration along straight paths is a closely related problem that also requires sensor placement~\cite{ArainSBL16}

\subsection{Related Work}

Building on prior GP approaches, \cite{SmithP05} presented an approach that leverages linear transformations on Gaussian process priors to model ill-posed inverse problems and reduce the computational complexity of Gaussian processes.  

\cite{LongiRSMRSHK20} addressed sensor placement for sparse view CT-scanning using the mutual information-based approach by~\cite{krauseSG08}. They leveraged the closed-form nature of Gaussian processes under linear transformations to extend the MI approach to handle the data-integrating sensor model of CT scanners. However, the method still relies on discrete optimization, which makes the approach computationally expensive and ill-suited for real-time applications.

\subsection{Linear and Non-linear Transformations}
\label{sec:transformations}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{An illustration of the sensor placement approach for sparse view CT scanning with fan beam projections. The expansion transformation maps each of the $m$ inducing points in the point parametrization to $p$ points in the FoV parametrization to approximate each sensor's FoV, and the aggregation transformation aggregates the covariances corresponding to the $mp$ points to model the sensor's integrated observations.}
    \label{fig:overview}
\end{figure*}

We now generalize our approach to handle sensors with non-point FoV and integrated observations. Although such sensor models have been attempted in prior work, our sensor placement approach's computational efficiency allows us to address significantly larger problems. As an illustrative example, we consider the problem of sensor placement for sparse view computed tomography (CT)~\cite{LongiRSMRSHK20}.

A third-generation fan beam CT scanner~\cite{Zeng17}  projects X-ray beams that fan out at a fixed angle~(Figure~\ref{fig:overview}). On the opposite side of the projector, a sensor array captures data integrated along each beam and encoded by the received X-ray intensity. The projector and sensor array pair rotate around a circular area of interest, and the collected data is then used to reconstruct the underlying spatially resolved data. Being able to compute informative sensor placements efficiently is especially useful when the region of interest is a sub-region of the observation space (e.g., if we only need to scan a specific organ), as we will be able to optimize the sensor placements in real-time, thereby reducing the amount of harmful X-ray exposure to patients while also retaining reconstruction quality.

\subsection{experiments}

We now demonstrate our sensor placement approach for sensors with non-point FoV and integrated observations. We do this by considering the sensor placement for the sparse view CT scanning problem~\cite{LongiRSMRSHK20}.  We used the whole observation space as the region of interest. We computed the solution sensor placements for 5 to 75 sensors (in increments of 10) using our approaches (with $p$ set to 20) and the mutual information-based approach presented in~\cite{LongiRSMRSHK20} as a baseline. We present the RMSE scores of the CT scan dataset reconstructions obtained using the solution sensor placement locations, and the sensor placement algorithm runtimes in Figure~\ref{fig:ct-rmse} and Figure~\ref{fig:ct-time}, respectively. Further technical details of the experiment are presented in the appendix.

Our results show that our approaches are significantly faster (up to 53 times) while maintaining the reconstruction quality obtained using the computationally intensive MI-based approach. In the Greedy-SGP case, the method is still faster than the MI approach despite using a greedy optimization method. Also, the Continuous-SGP and Discrete-SGP approaches take a fraction of the computation time of the baseline MI approach and take approximately constant time with increasing number of sensing locations.

\subsection{CT Scan dataset experiment details}

We used the COVID-19 CT scan dataset which contains lung scans from 10 patients, with each containing 301 slices~\cite{Jun20} to benchmark our sparse view CT scan sensor placements. We used a fan beam CT projection~\cite{Zeng17} with 750 detectors with a width of $2$. The source projection and the detector distance were set to $400$. We used filter back projection~\cite{Zeng17} from the ASTRA Toolbox~\cite{AarlePBABBS15} to generate our reconstructions using the data from only the placement locations. The kernel parameters were learned from phantom CT images.

\begin{table}[!htbp]
\begin{center}
\begin{tabular}{ |c|c c c c| }
\hline
\# Sensors & MI & Greedy-SGP & Discrete-SGP & Continuous-SGP \\
\hline
5 & 0.2569 & 0.2527 & 0.2613 & 0.2610 \\
15 & 0.1804 & 0.1764 & 0.1851 & 0.1856 \\
25 & 0.1431 & 0.1408 & 0.1424 & 0.1428 \\
35 & 0.1194 & 0.1194 & 0.1210 & 0.1216 \\
45 & 0.1046 & 0.1050 & 0.1056 & 0.1058 \\
55 & 0.0934 & 0.0940 & 0.0950 & 0.0936 \\
65 & 0.0850 & 0.0865 & 0.0841 & 0.0836 \\
75 & 0.0775 & 0.0793 & 0.0796 & 0.0796 \\
\hline
\end{tabular}
\caption{RMSE vs number of sensors for the CT scan dataset (lower is better).}
\end{center}
\end{table}

\begin{table}[!htbp]
\begin{center}
\begin{tabular}{ |c|c c c c| }
\hline
\# Sensors & MI & Greedy-SGP & Discrete-SGP & Continuous-SGP \\
\hline
\hline
5 & 0.1021 & 0.0973 & 0.0932 & 0.0934 \\
15 & 0.1475 & 0.1487 & 0.1438 & 0.1426 \\
25 & 0.1960 & 0.1974 & 0.1993 & 0.1984 \\
35 & 0.2323 & 0.2387 & 0.2317 & 0.2304 \\
45 & 0.2700 & 0.2696 & 0.2685 & 0.2675 \\
55 & 0.3029 & 0.2996 & 0.3014 & 0.3025 \\
65 & 0.3308 & 0.3266 & 0.3351 & 0.3354 \\
75 & 0.3592 & 0.3541 & 0.3569 & 0.3555 \\
\hline
\end{tabular}
\caption{SSIM vs number of sensors for the CT scan dataset (higher is better).}
\end{center}
\end{table}

\begin{table}[!htbp]
\begin{center}
\begin{tabular}{ |c|c c c c| }
\hline
\# Sensors & MI & Greedy-SGP & Discrete-SGP & Continuous-SGP \\
\hline
5 & 1125.9375 & 57.1025 & 4.0282 & 3.1066 \\
15 & 3102.5137 & 318.3406 & 13.1679 & 13.0909 \\
25 & 5066.4228 & 968.3583 & 35.8298 & 35.7661 \\
35 & 7038.7364 & 2160.8199 & 67.9413 & 67.8967 \\
45 & 9024.9766 & 3997.4588 & 96.5101 & 96.8211 \\
55 & 11048.5689 & 6616.1409 & 135.8416 & 131.0395 \\
65 & 13111.3387 & 10166.6850 & 219.5241 & 218.0974 \\
75 & 15341.4043 & 14624.4529 & 295.5247 & 295.7489 \\
\hline
\end{tabular}
\caption{Runtime vs number of sensors for the CT scan dataset (lower is better).}
\end{center}
\end{table}
